Gaia-ESO Survey: massive stars in the Carina Nebula. II. The spectroscopic analysis of the O-star population

The new census of massive stars in the Carina nebula reveals the presence of 54 apparently single O-type stars in the Car OB1 association, an extremely active star-forming region which hosts some of the most luminous stars of the Milky Way. A detailed spectroscopic analysis of the currently most complete sample of O-type stars in the association can be used to inspect the main physical properties of cluster members and test evolutionary and stellar atmospheres models. We perform quantitative spectroscopic analysis for the most complete sample of apparently single O-type stars in Car OB1 with available spectroscopic data. From the high-resolution GES and OWN spectra we obtain a reliable distribution of rotational velocities for a sample of 37 O-type stars. It shows a bimodal structure with a low velocity peak at 60 km s$^{-1}$ and a short tail of fast rotators reaching 320 km s$^{-1}$. We also perform quantitative spectroscopic analysis and derive effective temperature, surface gravity and He abundance for a sample of 47 O-type stars, now including further stars from GOSSS database. Radii, luminosities, and spectroscopic masses were also determined using $Gaia$ astrometry. We create the Hertzsprung-Russell Diagram to inspect the evolutionary status of the region and confirm the lack of stars close to the Zero Age Main Sequence (ZAMS) between $\sim$35 -- 55 M$_\odot$. We confirm a very young population with an age distribution peaking at 1 Myr, some stars close or even on the ZAMS, and a secondary peak at 4 -- 5 Myr in the age distribution. We confirm the youth of Trumpler 14, which is also the only cluster not showing the secondary peak. We also find a clear trend to evolutionary masses higher than derived spectroscopic masses for stars with evolutionary mass below 40 M$_{\odot}$.

==> table_fast.tex <==
\begin{table*}
\caption{Rotational velocities for the (very) fast B-type rotators analyzed in this work and {\it Gaia}~EDR3 proper motions.}
\label{table_fast}
\centerline{
\tiny
\addtolength{\tabcolsep}{-1mm}
\begin{tabular}{llllcccccl}
\hline
\hline
Name          &   SpT & LC & qual.  &   Spectral source  &   Line  &  $v\sin i$ [km s^{-1}]  & $\mu_\alpha$ [mas] & $\mu_\delta$ [mas] &  Notes \\   

\hline

HD 93 056                           &   B1:   &  V:  &   n    &       -            &  Si\,{\sc iii}  &  -              &  -   &   -  &    - \\
HD 93 249 B                         &   B0.2  &  V   &  (n)   &       -            &  Si\,{\sc iii}  &  -              &  -   &   -  &    - \\
HDE 303 300                         &   B0.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\
HD 93 097                           &   B0.2  &  V:  &   n    &                    &                 &                 &      &      &      \\
CPD -59 2593                        &   B1:   &  V   &  nn    &                    &                 &                 &      &      &      \\
ALS 15 205                          &   B0.2  &  V   &  (n)   &                    &                 &                 &      &      &      \\
HDE 305 533                         &   B0.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\
HD 93 249 C                         &   B1.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\
CPD -58 2657                        &   B0.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\              
CPD -59 2632                        &   B0.5  &  V   &   n    &                    &                 &                 &      &      &      \\              
CPD -59 2541                        &   B1.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\              
CPD -59 2616                        &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\              
2MASS J10441242-5934091             &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\              
2MASS J10435413-5918244             &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\              
ALS 15 248                          &   B1.5  &  V   &  nn    &                    &                 &                 &      &      &      \\              
HSB2012-3192                        &   B2:   &  V   &  ne    &                    &                 &                 &      &      &      \\               
CPD -59 2618                        &   B1:   &  V   &  (n)   &                    &                 &                 &      &      &      \\               
ALS 19 733                          &   B1    &  V   &  (n)   &                    &                 &                 &      &      &      \\     
2MASS J10441879-5951490             &   B1.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\    
2MASS J10443223-5933592             &   B2:   &  V   &   n    &                    &                 &                 &      &      &      \\    
HD 93 129 C                         &   B0.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\    
ALS 16 082                          &   B0.7  &  V   &  (n)   &                    &                 &                 &      &      &      \\    
2MASS J10454701-6000271             &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\    
2MASS J10451588-5929563             &   B2    &  IV  &   n    &                    &                 &                 &      &      &      \\ 
2MASS J10422722-6000052             &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                         
2MASS J10452314-5940033             &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                         
2MASS J10433865-5934444             &   B0.7: &  V   &  nn    &                    &                 &                 &      &      &      \\                        
2MASS J10435207-5932401             &   B2    &  V   &  (n)   &   GES- Giraffe     &  He\,{\sc i}    &    422          &      &      &      \\                        
ALS 19 747                          &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\                        
2MASS J10435198-6010368             &   B2.5  &  V   &   n    &                    &                 &                 &      &      &      \\
HSB2012-3545                        &   B1.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\                        
2MASS J10434797-6001201             &   B2.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\                        
2MASS J10443829-6005449             &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                        
2MASS J10454824-5922041             &   B2.5  &  V   &   n    &                    &                 &                 &      &      &      \\                        
HSB2012-3416                        &   B2.5: &  V   &  nn    &                    &                 &                 &      &      &      \\                        
2MASS J10442894-5943473             &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\ 
ALS 16 078                          &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\                        
2MASS J10450836-5938475             &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                        
2MASS J10430420-5948591             &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                        
2MASS J10444235-5922029             &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                        
2MASS J10444726-5928154             &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                        
Gaia ED3 5 350 302 097 055 370 496  &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                        
2MASS J10443591-5923356             &   B2.5  &  V   &   n    &                    &                 &                 &      &      &      \\       
2MASS J10460277-5950192             &   B2:   &  V   &  nnn   &                    &                 &                 &      &      &      \\                         
HSB2012-3314                        &   B2.5: &  V   &  nn    &                    &                 &                 &      &      &      \\                         
2MASS J10443822-5943056             &   B2    &  V   &  nnn   &                    &                 &                 &      &      &      \\   
2MASS J10451297-5946059             &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\                                     
Gaia ED3 5 350 388 683 629 610 752  &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\                                     
2MASS J10450792-593911              &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\                                     
HSB2012-1498                        &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                                     
2MASS J10435501-5936242             &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                                     
2MASS J10444208-5926353             &   B2:   &  V   &  nnn   &                    &                 &                 &      &      &      \\                                     
2MASS J10443769-5929316             &   B2.5  &  V   &   n    &                    &                 &                 &      &      &      \\ 
2MASS J10464886-5950409             &   B1.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\                                    
2MASS J10453254-5942359             &   B2:   &  V   &  nnn   &                    &                 &                 &      &      &      \\                                    
2MASS J10440866-5933488             &   B2:   &  V   &  nnn   &                    &                 &                 &      &      &      \\                                    
2MASS J10454060-5937041             &   B2:   &  V   &  nn    &                    &                 &                 &      &      &      \\
2MASS J10445602-5938530             &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\                                   
2MASS J10440683-5936116             &   B2    &  V   &  nnn   &                    &                 &                 &      &      &      \\                                   
2MASS J10434798-5933590             &   B2    &  V   &   n    &                    &                 &                 &      &      &      \\                                   
2MASS J10434580-5934359             &   B2:   &  V   &  nnn   &                    &                 &                 &      &      &      \\                                   
2MASS J10445837-5932062             &   B2.5  &  V   &   n    &                    &                 &                 &      &      &      \\                                   
2MASS J10442945-5933437             &   B2:   &  V   &  nnn   &                    &                 &                 &      &      &      \\                                   
2MASS J10460257-5957372             &   B2:   &  V   &   ne   &                    &                 &                 &      &      &      \\                                   
2MASS J10452056-5942212             &   B2:   &  V   &  nne   &                    &                 &                 &      &      &      \\
2MASS J10444710-5939201             &   B2    &  V   &  nn    &                    &                 &                 &      &      &      \\                                   
HSB2012-3526                        &   B2    &  V   &  (n)   &                    &                 &                 &      &      &      \\                                   
2MASS J10452415-5942313             &   B2.5: &  V   &  nn    &                    &                 &                 &      &      &      \\                                   
2MASS J10435009-5947024             &   B2.5  &  V   &  (n)   &                    &                 &                 &      &      &      \\                                    
HDE 305 535                         &   B4    &  III  &  (n)   &                    &                 &                 &      &      &      \\                                                                      
\hline
\multicolumn{10}{l}{O\,{\sc iii}: O\,{\sc iii}~5592, Si\,{\sc iii}: Si\,{\sc iii}~4552, He\,{\sc i}: He\,{\sc i}~4387,4471,4713, He\,{\sc ii}: He\,{\sc ii}~4542}
\end{tabular}
\addtolength{\tabcolsep}{1mm}
}
\end{table*}

